Diversified Node Sampling based Hierarchical Transformer Pooling for Graph Representation Learning

Graph pooling methods have been widely used on downsampling graphs, achieving impressive results on multiple graph-level tasks like graph classification and graph generation. An important line called node dropping pooling aims at exploiting learnable scoring functions to drop nodes with comparatively lower significance scores. However, existing node dropping methods suffer from two limitations: (1) for each pooled node, these models struggle to capture long-range dependencies since they mainly take GNNs as the backbones; (2) pooling only the highest-scoring nodes tends to preserve similar nodes, thus discarding the affluent information of low-scoring nodes. To address these issues, we propose a Graph Transformer Pooling method termed GTPool, which introduces Transformer to node dropping pooling to efficiently capture long-range pairwise interactions and meanwhile sample nodes diversely. Specifically, we design a scoring module based on the self-attention mechanism that takes both global context and local context into consideration, measuring the importance of nodes more comprehensively. GTPool further utilizes a diversified sampling method named Roulette Wheel Sampling (RWS) that is able to flexibly preserve nodes across different scoring intervals instead of only higher scoring nodes. In this way, GTPool could effectively obtain long-range information and select more representative nodes. Extensive experiments on 11 benchmark datasets demonstrate the superiority of GTPool over existing popular graph pooling methods.

==> tables/ogb_res.tex <==
\begin{table}
  \caption{Test performance (ROC-AUC) on 4 benchmarks from OGB. The shown results are mean ($\%$) and deviation ($\%$) over 10 different runs.
  The best results appear in bold. 
  }
  \label{tab:ogb_res}
  \setlength\tabcolsep{1.4mm}{
	\scalebox{0.75}{
  \begin{tabular}{lcccc}
    \toprule
    Method & HIV & TOX21 & TOXCAST & BBBP\\
    % Metric & Accuracy & Accuracy & Accuracy\\
    \midrule
    GCN & 76.81 $\pm$ 1.01 & 75.04 $\pm$ 0.80 & 60.63 $\pm$ 0.51 & 65.47 $\pm$ 1.83 \\
    GIN & 75.95 $\pm$ 1.35 & 73.27 $\pm$ 0.84 & 60.83 $\pm$ 0.46 & 67.65 $\pm$ 3.00 \\
    \midrule
    Set2Set &  73.42 $\pm$ 2.34 & 73.42 $\pm$ 0.67 & 59.76 $\pm$ 0.65 & 64.43 $\pm$ 2.16 \\
    SortPool & 71.82 $\pm$ 1.63 & 69.54 $\pm$ 0.75 & 58.69 $\pm$ 1.71 & 65.98 $\pm$ 1.70 \\
    DiffPool & 75.64 $\pm$ 1.86 & 74.88 $\pm$ 0.81 & 62.28 $\pm$ 0.56 & 68.25 $\pm$ 0.96 \\
    $\mathrm{SAGPool}_{g}$ & 74.56 $\pm$ 1.69 & 71.10 $\pm$ 1.06 & 59.88 $\pm$ 0.79 & 65.16 $\pm$ 1.93 \\
    $\mathrm{SAGPool}_{h}$ & 71.44 $\pm$ 1.67 & 69.81 $\pm$ 1.75 & 58.91 $\pm$ 0.80 & 63.94 $\pm$ 2.59 \\
    TopKPool  & 72.27 $\pm$ 0.91 & 69.39 $\pm$ 2.02 & 58.42 $\pm$ 0.91 & 65.19 $\pm$ 2.30 \\
    MincutPool & 75.37 $\pm$ 2.05 & 75.11 $\pm$ 0.69 & 62.48 $\pm$ 1.33 & 65.97 $\pm$ 1.13 \\
    StructPool & 75.85 $\pm$ 1.81 & 75.43 $\pm$ 0.79 & 62.17 $\pm$ 0.61 & 67.01 $\pm$ 2.65  \\
    ASAP & 72.86 $\pm$ 1.40 & 72.24 $\pm$ 1.66 & 58.09 $\pm$ 1.62 & 63.50 $\pm$ 2.47 \\
    HaarPool & - & - & - & 66.11 $\pm$ 0.82 \\
    GMT & 77.56 $\pm$ 1.25 & 77.30 $\pm$ 0.59 & \bf{65.44} \textbf{$\pm$} \bf{0.58} & 68.31 $\pm$ 1.62  \\
    \midrule
    %\name(ours) & $\mathbf{82.73 \pm 1.45}$ & $\mathbf{81.64 \pm 2.21}$ & $\mathbf{81.80 \pm 2.24}$ \\
    \bf{\name} & 77.94 $\pm$ 0.46 & 77.32 $\pm$ 0.12 & 65.34 $\pm$ 0.87 & 70.15 $\pm$ 0.29 \\
    \bf{\vname} & \bf{78.36} \textbf{$\pm$} \bf{0.35} & \bf{77.45} \textbf{$\pm$} \bf{0.56} & {65.18} {$\pm$} {1.12} & \bf{70.68} \textbf{$\pm$} \bf{0.33}\\
  \bottomrule
    \end{tabular}
}
}
\end{table}
